Persuading Farsighted Receivers in MDPs: the Power of Honesty

Bayesian persuasion studies the problem faced by an informed sender who strategically discloses information to influence the behavior of an uninformed receiver. Recently, a growing attention has been devoted to settings where the sender and the receiver interact sequentially, in which the receiver's decision-making problem is usually modeled as a Markov decision process (MDP). However, previous works focused on computing optimal information-revelation policies (a.k.a. signaling schemes) under the restrictive assumption that the receiver acts myopically, selecting actions to maximize the one-step utility and disregarding future rewards. This is justified by the fact that, when the receiver is farsighted and thus considers future rewards, finding an optimal Markovian signaling scheme is NP-hard. In this paper, we show that Markovian signaling schemes do not constitute the "right" class of policies. Indeed, differently from most of the MDPs settings, we prove that Markovian signaling schemes are not optimal, and general history-dependent signaling schemes should be considered. Moreover, we also show that history-dependent signaling schemes circumvent the negative complexity results affecting Markovian signaling schemes. Formally, we design an algorithm that computes an optimal and {\epsilon}-persuasive history-dependent signaling scheme in time polynomial in 1/{\epsilon} and in the instance size. The crucial challenge is that general history-dependent signaling schemes cannot be represented in polynomial space. Nevertheless, we introduce a convenient subclass of history-dependent signaling schemes, called promise-form, which are as powerful as general history-dependent ones and efficiently representable. Intuitively, promise-form signaling schemes compactly encode histories in the form of honest promises on future receiver's rewards.

==> pckgs.tex <==
\usepackage{amsfonts}
%\usepackage[numbers]{natbib}
\usepackage{multicol}
\usepackage{algorithm}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage[noend]{algpseudocode}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{thmtools}
%\usepackage{nicefrac, xfrac}
\usepackage{thm-restate}
\usepackage{lipsum}
\usepackage{amssymb }
\usepackage{mleftright}
\usepackage{color}
\usepackage{diagbox}
\usepackage{tikz}
\usepackage{wrapfig}
\usetikzlibrary{positioning,fit,calc,matrix,arrows,trees,backgrounds}
%\usepackage{accents}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{enumerate}
\usepackage[shortlabels]{enumitem}
\usepackage{bm}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{cleveref}

==> src/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%	justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%	\item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%	\item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%	\item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%%% END INSTRUCTIONS %%%


\begin{enumerate}
	
	
	\item For all authors...
	\begin{enumerate}
		\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
		\answerYes{}
		\item Did you describe the limitations of your work?
		\answerYes{The setting is based on precise assumptions. If those assumptions are not met then our techiques are not applicable.}
		\item Did you discuss any potential negative societal impacts of your work?
		\answerNA{Our work is mailny theoretical and thus the question does not apply.}
		\item Have you read the ethics review guidelines and ensured that your paper conforms to them?
		\answerYes{}
	\end{enumerate}
	
	
	\item If you are including theoretical results...
	\begin{enumerate}
		\item Did you state the full set of assumptions of all theoretical results?
		\answerYes{}
		\item Did you include complete proofs of all theoretical results?
		\answerYes{While all the main statements are contained in the main paper, all the proof are deferred to the appendix due to space constraints.}
	\end{enumerate}
	
	
	\item If you ran experiments...
	\begin{enumerate}
		\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
		\answerNA{}
		\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
		\answerNA{}
		\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
		\answerNA{}
		\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
		\answerNA{}
	\end{enumerate}
	
	
	\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
	\begin{enumerate}
		\item If your work uses existing assets, did you cite the creators?
		\answerNA{}
		\item Did you mention the license of the assets?
		\answerNA{}
		\item Did you include any new assets either in the supplemental material or as a URL?
		\answerNA{}
		\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
		\answerNA{}
		\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
		\answerNA{}
	\end{enumerate}
	
	
	\item If you used crowdsourcing or conducted research with human subjects...
	\begin{enumerate}
		\item Did you include the full text of instructions given to participants and screenshots, if applicable?
		\answerNA{}
		\item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
		\answerNA{}
		\item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
		\answerNA{}
	\end{enumerate}
	
	
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> src/dynamic_programming.tex <==
\section{Dynamic Programming}

In this section, we show how to compute an optimal and $\epsilon$-persuasive signaling scheme that can be represented compactly by a tuple $\bm{\phi} := ( \{ I_h \}_{h \in \Hi}, \{\phi_h\}_{h \in \Hi}, \{g_h\}_{h \in \Hi})$. As a first step, we consider a discretized set of continuation values $\mathcal{D}_\delta\coloneqq \{k \delta\}_{k \in \lfloor \frac{H}{\delta}\rfloor}$, where $\delta>0$ depends on the desired relaxation of the persuasiveness $\epsilon$.


Then, we consider a function of \[M_{\delta}:\Hi \times \Si \times I_\delta \rightarrow [0,H].\] Intuitively, $M_{\delta}(h,s,\iota)$ represents (an approximation of) the expected utility that can achieve the seller guaranteeing that the receiver's utility is at least $\iota$ in the path starting from $s$ at time $h$.

Our idea is to start build a function $M_\delta$ recursively exploiting an optimization oracle $\mathcal{O}_{\delta,\epsilon}$. The optimization oracle $\mathcal{O}_{\delta,\epsilon}$ with domain $\Hi \times \Si \times \mathcal{D}_\delta \times M$ returns a tuple $(\phi,g)$ with the following guarantees.

Given an $h$, $s$, and $\iota$, $(\phi,g)=\mathcal{O}_{\delta,\epsilon}(h,s,\iota,M)$ satisfies the following constraints:
\begin{subequations} \label{eq:conDP}
	\begin{align}
	\sum_{a \in \A} \sum_{\theta \in \Theta} \mu_h(\theta|s) \phi_h(a|s,\iota,\theta) \left[ r_h^\rec (s,a,\theta) + \sum_{s' \in \Si} p_h(s' | s,a,\theta)  g_h(s,a,\iota,s') \right] \geq \iota \\
	\sum_{\theta \in \Theta} \mu_h(\theta|s) \phi_h(a|s,\iota,\theta) \left[ r_h^\rec (s,a,\theta) + \sum_{s' \in \Si} p_h(s' | s,a,\theta)  g_h(s,a,\iota,s') \right] \geq \nonumber\\
	\sum_{\theta \in \Theta} \mu_h(\theta|s) \phi_h(a|s,\iota,\theta) \left[ r_h^\rec (s,a',\theta) + \sum_{s' \in \Si} p_h(s' | s,a',\theta)  \widehat V_{h+1}^{\rec}(s') \right]  - \delta 
\forall a \in \A, a' \in \A. 
	\end{align}
\end{subequations}

Moreover, the value of the signaling scheme
\[
M(h,s,\iota)\coloneqq\sum_{a \in \A}\sum_{\theta \in \Theta} \mu_h(\theta|s) \phi(a|\theta) \left[ r_h^\s (s,a,\theta) + \sum_{s' \in \Si} p_h(s' | s,a,\theta) M(h+1,s',g(a,s'))\right].
\]
is at least $\max\{OPT(h,s,M,\iota'),OPT(h,s,M,0)\}$, where $\iota'=\iota+\nu$ and $OPT(h,s,M,\bar \iota)$ is the solution of the following program:

\begin{subequations} %\label{Pr:DP}
	\begin{align}
&	\max_{\phi,g} \sum_{s',\theta,a} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)  \Big[ r_h^{\s} (s, a, \theta) + M(h+1,s',g(s',a)) \Big]\\
& \sum_{s',\theta,a} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta) \Big[ r_h^{\rec} (s, a, \theta) + g(s',a) \Big] \ge \bar \iota\\
& \sum_{s',\theta} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)  \Big[  r_h^{\rec} (s, a, \theta) + g(s',a)\Big] \\
&\quad \ge \sum_{s',\theta} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a',\theta) \Big[  r^{\rec}_{h} (s', a', \theta) + \hat V^{\rec}_{h + 1}(s') \Big] -\delta, \forall{a,a^\prime \in \A}
\end{align}
\end{subequations} 

Whenever Problem~\eqref{Pr:DP} is unfeasible, by assumption we set its value $OPT(\iota)$ to $-\infty$.




%
Algorithm~\ref{alg:DP} iteratively solves Problem~\eqref{Pr:DP} and build a signaling scheme $\bm{\phi} := ( \{ I_h \}_{h \in \Hi}, \{\phi_h\}_{h \in \Hi}, \{g_h\}_{h \in \Hi})$. We show that given an optimization oracle $\mathcal{O}_{\delta,\epsilon}$ Algorithm~\ref{alg:DP}  finds in polynomial time an almost persuasive and optimal signaling scheme.


\begin{theorem}
 Algorithm~\ref{alg:DP} returns an $\epsilon$-persuasive and optimal signaling scheme.
\end{theorem}

\begin{proof}
	By Lemma~\ref{lem:compact_pers} and Constraints~\eqref{eq:conDP}, the obtained signaling scheme is $\epsilon$-persuasive. \mat{In principio dimostrare che esiste una feasible.}
	%
	
	We are left to show that the signaling scheme achieves the optimal utility.
	%
	Let $\bm{\phi} := ( \{ I_h \}_{h \in \Hi}, \{\phi_h\}_{h \in \Hi}, \{g_h\}_{h \in \Hi})$ be an optimal succinct signaling scheme. 
	
	We denote with $V_{h}^{\s,\bm{\phi}}(s,\iota)$ and $V_{h}^{\rec,\bm{\phi}}(s,\iota)$ the expected value from node $s$ following signaling scheme $\iota$ at level $h$.
	We prove by induction that $M_{\epsilon,\delta}(h,s,\max\{\lfloor\iota - (\delta+ \nu) (H-h)\rfloor,0\}]\ge V_{h}^{\s,\bm{\phi}}(s,\iota)$.
	
	Consider a node $s$, a value $\iota$, and level $H$. Notice that  $OPT( \lfloor \iota \rfloor,h,s,M)\ge V_{h}^{\s,\bm{\phi}}(s,\iota)$ and $V_{h}^{\rec,\bm{\phi}}(s,\iota)$ by the definition of $OPT$. In particular, $\hat\phi$, $\hat g$ such that $\hat\phi(\cdot)= \phi_h(|s,\iota, \cdot)$ and $g=g_h(s,\cdot,\iota,	\cdot)$  is feasible for the problem defining $OPT$. By definition of oracle, OK with $\iota= \lfloor \iota \rfloor- \nu$.
	
	Consider a level $h$, node $s$, a value $\iota$. 
	Set $ \iota_1= \lfloor\iota\rfloor-(\nu+\delta)(H-h)$ and $ \iota_2= \lfloor\iota\rfloor-(\nu+\delta)(H-h+1)$. Consider a solution $\phi,g$ to $OPT$ such that same $\hat\phi= \phi_h(|s,\iota, \cdot)$ and $\hat g= \lfloor g_h(s,\cdot,\iota,	\cdot)-(H-h+1)(\nu+\epsilon)\rfloor$.
	Then,
	\begin{align}
	&\sum_{s',\theta,a} \mu_h(\theta| s) \hat \phi(a|\theta) p_h(s'|s,a,\theta)  \Big[ r_h^{\s} (s, a, \theta) + M(h+1,s',\hat g(s',a)) \Big] \ge \\
	&\sum_{s',\theta,a} \mu_h(\theta| s) \hat \phi(a|\theta) p_h(s'|s,a,\theta)  \Big[ r_h^{\s} (s, a, \theta) + V_{h}^{\s,\bm{\phi}}(s,\iota) \Big] 
	\end{align}
	
	Moreover,
		\begin{align}
	&\sum_{s',\theta,a} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta) \Big[ r_h^{\rec} (s, a, \theta) + g(s',a) \Big] \ge \iota_1 \\
	\end{align}
	and
			\begin{align}
	& \sum_{s',\theta} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)  \Big[  r_h^{\rec} (s, a, \theta) + g(s',a)\Big] \\
	&\quad \ge \sum_{s',\theta} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a',\theta) \Big[  r^{\rec}_{h} (s', a', \theta) + \hat V^{\rec}_{h + 1}(s') \Big] -\delta, \forall{a,a^\prime \in \A}
		\end{align}
	The end.
\end{proof}



\begin{lemma}
%	M is convex.
%	Given an $h \in [H]$, suppose that for each $s \in \Si$, and any distribution $\gamma \in \Delta_{\mathcal{D}_\epsilon}$, $M(h+1,s,\lceil\sum_{\iota} \gamma(\iota) \iota\rceil) \ge \sum_{\iota} \gamma(\iota) M(h+1,s,\iota)-\lambda$.
%	Then, for each $s\in \Si$ and distributions $\{\gamma_{a,s'}\}\in \Delta_{\mathcal{D}_\epsilon}^{|A|}$ for each $a \in A,s \in \Si$, letting $i^*_{a,s}=\lfloor\sum_{\iota} \gamma_{s',a}(\iota) \rfloor$.
For each $h,s$ and distribution $\Delta \in \mathcal{D}_\epsilon$, letting $i^*= \lfloor\sum_{\iota}\gamma(\iota) \iota\rfloor$
	\[  M(h,s,\iota^*) \ge \sum_{\iota} \gamma(\iota) M(h,s,\iota)-(\epsilon+ \nu) (H-h)  \]
\end{lemma}

\begin{proof}
	Suppose satisfied for level $h+1$. We show that it is satisfied for level $h$.
\end{proof}


\begin{algorithm}[t!]
	\caption{Dynamic Programming Algorithmic for computing an optimal and $\epsilon$-persuasive signaling scheme}
	\label{alg:DP}
	\begin{algorithmic}[t]
		\State initialize $\iota=0$
		\For{$h = H,\ldots, 1 $}
		\For{$s \in \Si $}
		\For{$\iota \in \mathcal{D}_\epsilon$}
		\State $(\phi,g)=\mathcal{O}_{\epsilon,\delta}(h,s,\iota)$
		\State $M(h,s,\iota)$ equal to the value of $(\phi,g)$
		\State $\phi_{h}(a|s,\theta,\iota)$ solution of $g$  for each $\theta$ and $\iota$
		\State $g_{h}(s,a,\iota,s')\gets x_a$ that is solution of $M_{\epsilon,\delta}(h,s,\iota)$ for each $a$
		\If  {$M[h,s,\iota]\ge 0$}, 
		\State $I_h(s)\gets  I_h(s)\cup \iota$
		\EndIf
		\EndFor
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}






==> src/hardness.tex <==

\section{Hardness}

In this section, we show that design a time-inhomogeneous policy that is $\epsilon$-IC is an NP-Hard problem.

Formally, we consider the following problem.

\begin{definition}[\textsc{ApxBP}$(\alpha,\epsilon)$]\label{def:probelm}
	%
	For any $\alpha,\epsilon > 0$, we define \textsc{ApxBP}$(\alpha,\epsilon)$ as the problem of finding, given an instance I as input, a constrained $\epsilon$-persuasive time-inhomogeneous signaling scheme such that has sender reward at least $\alpha \textnormal{OPT}$, where $\textnormal{OPT}$ is the reward of the optimal persuasive time-inhomogeneous signaling scheme.
\end{definition}
%

We show that there exists constant $\alpha<1$ and $\epsilon>0$ such that \textsc{ApxBP}$(\alpha,\epsilon)$ is NP-Hard.

We reduce from a promise version of vertex cover.
%
In particular, given a graph $(V,E)$, there exists an $\gamma>1$ such that it is NP-Hard to decide if there exists an vertex cover of size $k$ or if all the vertex cover has size at least $\gamma k$.


\begin{theorem}
	There exist two constants $\alpha<1$ and $\epsilon>0$ such that \textsc{ApxBP}$(\alpha,\epsilon)$ is NP-Hard.
\end{theorem}

\begin{proof}
	There set of states includes $s_0$, $s_1$, $s_2$ and $s_4$, a state $s_e$ for each $e \in E$, and a state $s_v$ for each $v \in V$.
	%
	In state $s_0$ there is a single state of nature $\theta_0$ and two actions $a_{0,1}$ and $a_{0,2}$.
	The transition function is such that  $p(s_3|s_0,a_{0,1}, \theta_0)=1$ while $p(s_e|s_0,a_{0,2}, \theta_0)=\frac{1}{|E|}$ for each $e \in E$. The rewards of the receiver are $r^\rec(s_1,a_{0,1},\theta_0)=1$ and $0$ otherwise. The rewards of the sender are always $0$.
	%
	In state $s_1$, there is a single state of nature $\theta_1$ and a single actions $a_{1}$. The transition function is such that  $p(s_2|s_1,a_{1}, \theta_1)=1$ and the rewards of the agents are always $0$.
	%
	In state $s_2$, there is a single state of nature $\theta_2$ and a single actions $a_{2}$. The transition function is such that  $p(s_v|s_2,a_{2}, \theta_2)=\frac{1}{|V|}$ for each $v \in V$. The rewards of the agents are always $0$.
	%	
	In state $s_e$, $e=(u,v)\in E$ there is a single state of nature $\theta_e$, and two actions  $a_{e,v}$ and $a_{e,u}$.
	The transition function is such that  $p(s_v|s_e,a_{e,v}, \theta_e)=1$ and $p(s_u|s_e,a_{e,u}, \theta_e)=1$. The rewards of the agents are $0$. 
	%
	In state $s_v$ there are two states of nature $\theta_{v,1}$ and $\theta_{T,2}$, three actions $a_{T,1}$, $a_{T,2}$, and $a_{T,3}$.
	The transition function is such that  $p(s_3|S_T,a,\theta)=1$ for each $a$ and $\theta$. The rewards of the receiver are $r^\rec(s_T,a_{T,1},\theta_{T,1})=1$, $r^\rec(s_T,a_{T,2},\theta_{T,2})=1$, $r^\rec(s_T,a_{T,3},\theta_{T,1})=r^\rec(s_T,a_{T,1},\theta_{T,2})=\frac{1}{2}$ and $0$ otherwise. 
	The rewards of the sender are is $1$ if the receiver plays $a_{T,3}$ and $0$ otherwise.
	
	The initial distribution over the states is $\beta$ such that $\beta(s_0)=\frac{1}{2}$ and $\beta_{s_e}=\frac{1}{2m}$.
	
	The time horizon $H=3$.
	
	\paragraph{Completeness.}
	Suppose that there exists an set cover $V^*$ of size $k$.
	Consider the signaling scheme such that $\phi_{s_0}(a_{0,2}|\theta_0)=1$.
	 $\phi_{s_e}(a_{e,T}|\theta_e)=1$ for a $v$ such that $v \in e$.
	 Moreover, $\phi_{s_1}(a_{1}|\theta_1)=1$ and $\phi_{s_2}(a_{2}|\theta_2)=1$.
	 $\phi_{s_e}(a_{e,T}|\theta_e)=1$ for a $v$ such that $v \in e$.
	 Finally,  $\phi_{s_v}(a_{v,1}|\theta_{v,1})=1$, $\phi_{s_v}(a_{v,2}|\theta_{v,2})=1$ if $v \in V^*$ and $\phi_{s_v}(a_{v,3}|\theta_1)= \phi_{h,s_T}(a_{v,3}|\theta_2)=1$ otherwise.
	 
	We show that the signaling scheme is IC.
	In node $s_0$, the expected utility of following the recommendations is $1$, while the utility deviating on action $a_{0,2}$ is the same.
	
	In a node $s_1$ and $s_2$, only one action
	
	In a node $s_v$, not deviating.
	
	Hence, the total sender utility is $\frac{1}{2}(1-\frac{k}{|V|})+ 1-\frac{k}{|V|}$.
	
	\paragraph{Soundness.}
	Suppose all the vertex cover have size at least $\alpha k$. 
	
	First, notice that the sender has to recommend $a_{0,2}$ in node $s_{0}$ otherwise the utility is at most $\frac{1}{2}$.
	Then, suppose that for $l$ nodes $s_e$ the utility from there on is smaller than $1-\delta$. This implies that the expected utility following the recommendation is $s_0$ is at most $l/|E|(1-\delta)+ (1-l/|E|) \ge 1-\epsilon$.
	This implies that $l\le |E| \epsilon/\delta$.
	%Hence, there are at most $l$ nodes $s_v$ with utility smaller than $1-\delta$.
	
	Let $\hat V$ be such that the receiver's utility is at least $1-\delta$. 
	Then, $|\hat V|\ge \beta k-l$. Suppose otherwise. Then, there exists a set $\hat V< \beta k-l$ that covers at least $|E|-l$ edges. Hence a set of size $\beta k$ covers all the edges.
	
	$|\hat V|\ge\beta k-l \ge \beta k- |E| \epsilon/\delta	\ge \rho k$.
	
	In all the nodes $s_v$, $v \in \hat V$ the utility of the sender is at most $2\delta$  ( $\frac{1}{2} x+ 1 (1-x) \ge 1-\delta$ implying $x\le 2\delta$.)
	
	Hence, the total utility is $\frac{1}{2} +\rho \frac{k}{v} 2 \delta+ (1-\rho \frac{k}{v})$.
	
	
	 
	
	
	

\end{proof}

==> src/recursive_step.tex <==
\section{How to compute efficiently the recursive step}


We can modify the program introducing a variable $z_{s',a,\iota'}$ (representing $ \sum_{\theta}\mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta) x_{s',a}(\iota')$) and the constraint 
\[\sum_{\iota \in \mathcal{D}_\epsilon} z_{a,\iota}= \sum_{\theta}\mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)).\]
In the following, we show how to recover the original variables $x$ from $z$.
Moreover, we relax the constraints on $x_{s',a}$ to $x_{s',a} \in \Delta_{\mathcal{D}_\epsilon} \forall s \in \Si, a \in A$.
We obtain the following LP.

\begin{subequations} \label{Pr:DP2}
	\begin{align}
	&\underset{\substack{\phi:\Theta\rightarrow \Delta_A,\\
			z_{s',a,\iota} \in \mathbb{R}_+ \forall s' \in \Si, a \in A, \iota \in I_\epsilon}}{\text{ max}} \sum_{s',\theta,a} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)   r_h^{\s} (s, a, \theta) + \sum_{\iota' \in \mathcal{D}_\epsilon} z_{s',a,\iota'} M(h+1,s,\iota')  \\
	& \sum_{s',\theta,a} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)  r_h^{\rec} (s, a, \theta) + \sum_{\iota' \in \mathcal{D}_\epsilon} z_{s',a,\iota'} \iota'  \ge \iota\\
	& \sum_{s',\theta} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)    r_h^{\rec} (s, a, \theta) + \sum_{\iota'} z_{s',a,\iota'} \iota'  \\
	&\quad \ge \sum_{s',\theta} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a',\theta) \Big[  r^{\rec}_{h} (s, a', \theta) + \hat V^{\rec}_{h + 1}(s') \Big] -\delta, \forall{a,a^\prime \in \A}\\
	&\sum_{\iota \in \mathcal{D}_\epsilon} z_{s',a,\iota}= \sum_\theta \mu_h (\theta|s) p_h(s'|s,a,\theta) \phi(a|\theta) \forall s' \in \Si, a \in A
	\end{align}
\end{subequations}

This can be solved in polynomial time.
%
Then, we obtain a solution to Program~\eqref{Pr:DP} obtaining a solution $(\phi,x)$ from $(\phi,z)$ and then rounding the variable $x$.
%
\begin{lemma}
	Given a feasible solution to LP~\eqref{Pr:DP2}, there exists a feasible solution to Program~\eqref{Pr:DP} with at least the same value. Moreover, this solution can be recover in polynomial time.
\end{lemma}

\begin{proof}
Let $(\phi,z)$ be a feasible solution to LP~\eqref{Pr:DP2}. Consider a solution to Program~\eqref{Pr:DP} such that $x_{s',a}(\iota')= \frac{z_{a,\iota}}{\sum_{\theta}\mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)}$ for each $s' \in \Si$, $a \in A$, and $\iota\in \mathcal{D}_\epsilon$. Moreover, if $\sum_{\theta}\mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)=0$ we set $x_{s',a}(0)=1$ (any value is fine but we need to satisfy the simplex constraint).

We show that if $(\phi,x)$ is a feasible solution to Program~\eqref{Pr:DP}. In particular, it is easy to see that all the constraints are satisfied.

Moreover, $x_{s',a} \in \Delta_{\mathcal{D}_\epsilon}$.

\end{proof}


The second component is the rounding of the solution $\phi,x_{s',a}$.


we need this auxiliary lemma.


\begin{lemma}
	Given an $h \in [H]$, suppose that for each $s \in \Si$, and any distribution $\gamma \in \Delta_{\mathcal{D}_\epsilon}$, $M(h+1,s,\lceil\sum_{\iota} \gamma(\iota) \iota\rceil) \ge \sum_{\iota} \gamma(\iota) M(h+1,s,\iota)-\lambda$.
	Then, for each $s\in \Si$ and distributions $\{\gamma_{a,s'}\}\in \Delta_{\mathcal{D}_\epsilon}^{|A|}$ for each $a \in A,s \in \Si$, letting $i^*_{a,s}=\lfloor\sum_{\iota} \gamma_{s',a}(\iota) \rfloor$.
	\[  \sum_{s',\theta,a} \mu_h(\theta| s) \phi(a|\theta) p_h(s'|s,a,\theta)   r_h^{\s} (s', a, \theta) + \iota^*_{s,a} M(h+1,s',\iota^*_{a,s'}) \ge \sum_{\iota} \gamma(\iota) M(h+1,s,\iota)-\lambda -\epsilon  \]
\end{lemma}

\begin{proof}
	The utility decreases by at most $\epsilon$. We show that 
\end{proof}

\begin{lemma}
	Given a feasible solution to Program~\eqref{Pr:DP} with $x_{s',a}\in \Delta_{\mathcal{D}_\epsilon}$, there exists a integer feasible solution to ? with at least the same value.
\end{lemma}

\begin{proof}
	For each $s'$ and $a$, we let $\iota^*=\sum_{\iota'}x_{s',a}(\iota') \iota'$.
	Then we set $x=\bar\iota$, where $\bar \iota$ is the largest in $\mathcal{D}_\epsilon$ smaller than $\iota^*$.
\end{proof}
%\begin{align*}
%& \underset{\phi:\Theta\rightarrow \Delta_A, z_{s,a,\theta,\iota}\ge 0}{\text{max}} \sum_{s,\theta,a} \mu_h(\theta| s_h) \ p_h(s|s_h,a,\theta)  \Big[ \phi(a | \theta) r_h^{\s} (s_h, a, \theta) +  \sum_{\iota} z_{s,a,\theta,\iota} M[h+1,s,\iota] \Big] \\
%& \sum_{s,\theta,a} \mu_h(\theta| s_h) p_h(s|s_h,a,\theta)  \Big[ \phi (a| \theta) r_h^{\rec} (s_h, a, \theta) +  \sum_{\iota} z_{s,a,\theta,\iota} \iota \Big] \ge \alpha\\
%& \sum_{s,\theta} \mu_h(\theta| s_h)  p_h(s|s_h,a,\theta)  \Big[ \phi (a| \theta) r_h^{\rec} (s_h, a, \theta) +   \sum_{\iota} z_{s,a,\theta,\iota} \iota \Big]\\
%& \quad \ge \sum_{s,\theta} \mu_h(\theta| s_h) \phi(a|\theta) p_h(s|s_h,a',\theta) \Big[  r^{\rec}_{h} (s_h, a', \theta) + \hat V^{\rec}_{h + 1}(s) \Big], \forall{a,a^\prime \in \A}\\
%&\sum_{\iota} z_{s,a,\theta,\iota}= \phi(a|\theta)
%\end{align*}


%Once we solve this LP, we can recover a solution setting $x_{s,a,\theta}(\iota)= z_{s,a,\theta,\iota}/\phi(a|\theta)$. Notice that it is always well-defined.
%This concludes the recursive step.










%\begin{proof}
%	Let $\phi^*$ be the optimal signaling scheme. We show inductively that for each $h,s,\tau$, given $\alpha=V^R(\phi_{h,s,\tau})$ the value of the cell is at least  $M[h,s,\alpha]\ge V^S(\phi_{h,s,\tau})$.
%	Given $\phi_\tau$, we show that the solution $\phi= \phi_\tau $ and  $x_{s',a,\theta} = V^r (\phi_\tau \oplus (a, \theta,s'))$ is feasible to $Find(h,s,\alpha-\epsilon)$.
%	Applying inductively, we get that the value of the computed signaling scheme is optimal.
%	
%	We are left to show that the signaling scheme is indeed $f(\epsilon)$-persuasive.
%	
%\end{proof}




\begin{corollary}
	Polynomial time algorithm.
\end{corollary}







==> src/trash.tex <==
\section{tentativo matteo}

LP to find optima

For each node $\phi_\theta( \cdot)$.

utility of deviating on a' given $s,h,\theta$  is a number.
\[
\hat V_h^\rec(s,h,\theta,a').
\]

utility of following is 
\[
 V_h^\rec(s,h,\theta,a)= r^\rec_{h}(s,a,\theta) + \sum_{s',\theta',a'} p_{h}(s'|s,a,\theta) \mu_{s',h+1}(\theta') \phi_\theta( a') V_h^\rec(s',h+1,\theta',a').
\]

utility of sender
\[V_h^S(s,h,\theta,a)=r^S_{h}(s,a,\theta) + \sum_{s',\theta',a'} p_{h}(s'|s,a,\theta) \mu_{s',h+1}(\theta') \phi_\theta( a') V_h^S(s',h+1,\theta',a')\]



\begin{align}
\max_{\phi}  & \sum_{\theta,a} \mu_{1,s_0}(\theta) \phi_{\theta}(a)V_h^S(s_0,1,\theta,a)\\
&s.t. \sum_{\theta \in \Theta} \mu_{s,h}(\theta) \phi_{\theta}(a) V_h^\rec(s,h,\theta,a)   \ge  \sum_{\theta \in \Theta} \mu_{s,h}(\theta) \phi_{\theta}(a) \hat V_h^\rec(s,h,\theta,a') \forall s,h,a,a'
\end{align}


\begin{align}
\max_{\phi}  & \sum_{\theta,a} \mu_{1,s_0}(\theta) \phi_{\theta}(a)V_h^S(s_0,1,\theta,a)+ \sum_{{s,h,a,a'}} \lambda_{s,h,a,a'} (\sum_{\theta \in \Theta} \mu_{s,h}(\theta) \phi_{\theta}(a) V_h^\rec(s,h,\theta,a) -\hat V_h^\rec(s,h,\theta,a'))\\
\end{align}

\section{Learning}

\ma{Che cosa learniamo? Solo le $p$ o anche le $r$? }


OLD
\subsection{Bayesian persuasion in MDP}\label{subsec:bpsdm}

We study \emph{Bayesian persuasion in MDP} (BPMDP) problems.
%
These extend the {Bayesian} persuasion framework~\citep{kamenica2011bayesian} to MDp problems by introducing an exogenous agent that acts as a \emph{sender} by issuing signals to the decision-making agent (the \emph{receiver}).
% introducing an exogenous agent in the SDM process that needs to persuade the agent to change its action, by sending signals to the agent. To mimic the Bayesian Persuasion nomenclature we will refer to the exogenous agent as the \emph{sender} and the agent that plays in the SDM as the \emph{receiver}.
%
%As customary in the literature, in BPSDM problems both agents know \ma{non li confodiamo così}the probability distributions $\mu_h$ of chance nodes in the underlying SDM problem.
%
By following the Bayesian persuasion terminology, the probability distributions $\mu_{s,h}\in\Delta(\Theta_{s,h})$ for each state $s$ and time $h$ are collectively referred to as the \emph{prior}.
%
Thus, the sender observes the realizations of random events occurring in the MDP problem and can partially disclose information to influence the receiver's behavior.
%
Moreover, the sender has their own utility function defined similar to the receiver's one, denoted as $v_{s,h}(a,\theta)$, and their goal is to commit to a publicly known \emph{signaling scheme} that maximizes their utility in expectation with respect to the prior, the signaling scheme, and the receiver's strategy.
%
%This is attained by sending signals to the receiver according to some \emph{signaling scheme}, which is selected beforehand by the sender and known to the receiver.

We focus on time-depended signaling schemes \textcolor{red}{terminologia per dire che dipendono solo dal nodo e time-step}.
Formally, a signaling scheme for the sender defines a probability distribution $\phi_{s,h} \in \Delta(\Signal_{s,h})$ at each tuple of state and time $(s,h)$, where $\Signal_{s,h}$ is a finite set of signals available at $h$.
%
Then, based on the signal $s \in \Signal_{s,h}$, the receiver computes a \emph{posterior} belief over over the states of natures and plays so as to maximize their expected utility in the MDP sub-problem that starts from $s,h$, taking into account the just acquired information.

%
% Given that SDM problems unfold in a tree structure, we assume that the sender can send a signal to the receiver each time an infoset is reached, before the receiver takes any action at that infoset.
%
% In particular, for every infoset $I \in \I$, a signalling scheme defines a probability distribution over signals available at $I$ as a function of the realizations of random events observed by the sender before reaching $I$.
% The sender then can send signals to the receiver, before the latter acts at some infoset $I$, by drawing them from the publicly known signalling scheme. 

As customary in these settings, a simple revelation-principle-style argument allows us to focus on signaling schemes that are \emph{direct} and \emph{persuasive}~\citep{kamenica2011bayesian, arieli2019private}.
%
In particular, a signaling scheme is direct if signals correspond to action recommendations, namely $\Signal_{s,h} = \A_{s,h}$ for all $s\in \Si,h\in \Hi$.
%
A direct signaling scheme is persuasive if the receiver is incentivized to follow action recommendations issued by the sender.
%
Moreover, we assume that, if the receiver does \emph{not} follow action recommendations at some decision node, then the sender stops issuing recommendations at nodes later reached during the SDM problem.
%
This is without loss of generality.
%
We refer to~\citep{von2008extensive, morrill2021hindsight} for a discussion on a similar problem in the field of correlation in sequential games.
